Neural Jump Stochastic Differential Equations

Many time series are effectively generated by a combination of deterministic continuous flows along with discrete jumps sparked by stochastic events. However, we usually do not have the equation of motion describing the flows, or how they are affected by jumps. To this end, we introduce Neural Jump Stochastic Differential Equations that provide a data-driven approach to learn continuous and discrete dynamic behavior, i.e., hybrid systems that both flow and jump. Our approach extends the framework of Neural Ordinary Differential Equations with a stochastic process term that models discrete events. We then model temporal point processes with a piecewise-continuous latent trajectory, where the discontinuities are caused by stochastic events whose conditional intensity depends on the latent state. We demonstrate the predictive capabilities of our model on a range of synthetic and real-world marked point process datasets, including classical point processes (such as Hawkes processes), awards on Stack Overflow, medical records, and earthquake monitoring.

==> paper/plan.tex <==
\section{Plan}
\begin{enumerate}
    \item \sout{We are going to implement our dynamics and inference algorithm in the neural ODE framework.}
    \item \sout{We plan to synthesize a discrete time event dataset using Hawkes process and test how well our model is able to capture the ground-truth mechanism. We will optimize the architecture of our model in this step.}
    \item We will benchmark the efficiency of our model and explore possible ways (code optimization, sampling, parallelization, etc) to speed it up.
    \item We plan to deploy our model on some real-world dataset for predicting the behavior of entities in the network, and compare with existing state-of-the-art methods.
    \item \sout{In the end, we will try to develop some theory about our model, such as the stationary point analysis of the learned differential equation.}
\end{enumerate}


\section{Questions to be Answered}
\begin{enumerate}
    \item How deep should the neural-blocks be?
    \item Are the learned parameters in one instance of the calculation transferable to another instance?
    \item \sout{Is maximizing the likelihood the right thing to do?}
    \item \sout{What is the correspondence to SGD batch sampling here?}
\end{enumerate}

%
